Towards Open-World Object-based Anomaly Detection via Self-Supervised Outlier Synthesis

Object detection is a pivotal task in computer vision that has received significant attention in previous years. Nonetheless, the capability of a detector to localise objects out of the training distribution remains unexplored. Whilst recent approaches in object-level out-of-distribution (OoD) detection heavily rely on class labels, such approaches contradict truly open-world scenarios where the class distribution is often unknown. In this context, anomaly detection focuses on detecting unseen instances rather than classifying detections as OoD. This work aims to bridge this gap by leveraging an open-world object detector and an OoD detector via virtual outlier synthesis. This is achieved by using the detector backbone features to first learn object pseudo-classes via self-supervision. These pseudo-classes serve as the basis for class-conditional virtual outlier sampling of anomalous features that are classified by an OoD head. Our approach empowers our overall object detector architecture to learn anomaly-aware feature representations without relying on class labels, hence enabling truly open-world object anomaly detection. Empirical validation of our approach demonstrates its effectiveness across diverse datasets encompassing various imaging modalities (visible, infrared, and X-ray). Moreover, our method establishes state-of-the-art performance on object-level anomaly detection, achieving an average recall score improvement of over 5.4% for natural images and 23.5% for a security X-ray dataset compared to the current approaches. In addition, our method detects anomalies in datasets where current approaches fail. Code available at https://github.com/KostadinovShalon/oln-ssos.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/coda.tex <==

\begin{table}
    \centering
    \begin{tabular}{|l||c|c|c|c|c|} \hline 
          k&  Dataset&  mAR&  AR50&  AR75& AR10\\ \hline 
          5&  &  &  9.5&  1.5& 1.6\\ \hline 
          20&  &  &  13.3&  3.5& 1.2\\ \hline 
          40&  &  &  2.5&  1.7& 0.6\\ \hline 
          100&  &  &  1.3&  0.2& 0.4\\ \hline
    \end{tabular}
    \caption{CODANOVELvos}
    \label{tab:CODA_NOVEL_vos
    }
\end{table}



\FloatBarrier
\begin{table}
    \centering
    \begin{tabular}{|l||c|c|c|c|c|} \hline 
          k&  Dataset&  mAR&  AR50&  AR75& AR10\\ \hline 
          5&  &  &  10.6&  1.3& 1.7\\ \hline 
          20&  &  &  10.7&  1.6& 1.4\\ \hline 
          40&  &  &  5.4&  0.5& 0.7\\ \hline 
          100&  &  &  15.1&  2.4& 1.8\\ \hline
    \end{tabular}
    \caption{CODANOVELffs}
    \label{tab:CODA_NOVEL_ffs
    }
\end{table}
\FloatBarrier

\FloatBarrier
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figures/coda.png}
\end{figure}
\FloatBarrier
text

==> tables/fishylaf.tex <==
\FloatBarrier
text
\begin{table*}[h!]
    \centering
    \begin{tabular}{|l||c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline  
          &&  &  \multicolumn{3}{|c|}{Pixel-level}&    &&\multicolumn{12}{|c|}{Component-level}\\ \hline  
          &&  &  \multicolumn{3}{|c|}{Anomaly scores}&    &&&  &  \multicolumn{3}{|c|}{$\tau$ = 0.25}&  \multicolumn{3}{|c|}{$\tau$ = 0.50}&  \multicolumn{3}{|c|}{$\tau$ = 0.75}& \\ \hline  
          &k& ep&AuPRC  &  FPR$_{95}$&$F_{1}$  &  k&ep&sIoU   &PPV   &FN   &FP   &$F_{1}$ &  FN   &  FP   &  $F_{1}$ &  FN   &  FP   &  $F_{1}$ & $\overline{F_{1}}$ \\ \hline  
          vos&20&37&  0.60&  62.3&  2.0&    5&8&\textbf{35.2}&  5.2& \textbf{90} &  1222& 10.3& \textbf{101}&  1231&  8.8& \textbf{113}  &  1233&  7.2& 8.9\\ \hline  
          vos-ffs&5&  11&  0.6&  71.6&  1.9&    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline 
    \end{tabular}
    \caption{FishyscapeLostnFound-val}
    \label{tab:my_label}
\end{table*}
\FloatBarrier
text
\FloatBarrier
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figures/fishylaf_val.png}
\end{figure}
\FloatBarrier
text

==> tables/laftestnoknown.tex <==
\FloatBarrier
text
\begin{table*}[h!]
    \centering
    \begin{tabular}{|l||c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline  
          &&  &  \multicolumn{3}{|c|}{Pixel-level}&    &&\multicolumn{12}{|c|}{Component-level}\\ \hline  
          &&  &  \multicolumn{3}{|c|}{Anomaly scores}&    &&&  &  \multicolumn{3}{|c|}{$\tau$ = 0.25}&  \multicolumn{3}{|c|}{$\tau$ = 0.50}&  \multicolumn{3}{|c|}{$\tau$ = 0.75}& \\ \hline  
          &k& ep&AuPRC  &  FPR$_{95}$&$F_{1}$  &  k&ep&sIoU   &PPV   &FN   &FP   &$F_{1}$ &  FN   &  FP   &  $F_{1}$ &  FN   &  FP   &  $F_{1}$ & $\overline{F_{1}}$ \\ \hline  
          vos&&&  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          vos-ffs&&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline 
    \end{tabular}
    \caption{LostnFoundTestNoKnown-val}
    \label{tab:my_label}
\end{table*}
\FloatBarrier
\FloatBarrier
text
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figures/laftestnoknown.png}
\end{figure}
\FloatBarrier

==> tables/results_ltdimaging.tex <==
\begin{table}[t]
\centering
\caption{Anomaly detection metrics for the LTDImaging dataset.}

\label{tab:ltdimaging_results}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{|l|cccccc|cccccc|}
\hline
 & \multicolumn{6}{|c|}{In-distribution Test Set} & \multicolumn{6}{|c|}{OoD Test Set} \\ \hline
\textbf{Method} & \textbf{AR@1} & \textbf{AR@10} & \textbf{AR@100} & \textbf{AR@S} & \textbf{AR@M} & \textbf{AR@L} & \textbf{AR@1} & \textbf{AR@10} & \textbf{AR@100} & \textbf{AR@S} & \textbf{AR@M} & \textbf{AR@L} \\ \hline
SIREN \cite{du2022siren}  &5.9&	34.2&	\textbf{52.5}&	\textbf{51.6}&	75.1&	- & 0.0&0.0&0.0&0.0&0.0&0.0\\
VOS \cite{du2022vos}   &\textbf{6.0}	&\textbf{34.3}&	\textbf{52.5}&	\textbf{51.6}&	75.1&	-&	0.0&0.0&0.0&0.0&0.0&0.0\\
FFS  \cite{kumar2023normalizing}  &\textbf{6.0}	&34.2&	\textbf{52.5}&	\textbf{51.6}&	\textbf{75.6}&	-&0.0&0.0&0.0&0.0&0.0&0.0\\
% OLN-VOS Box $k=5$ (Ours) &3.8	&16 	&18.5	&16.4	&71.0	&-& \textbf{8.2}&	10.4&	15.7&	0.1&	14.9&	55.1\\
% OLN-VOS Box $k=10$(Ours) &3.6	&15.5	&17.8	&15.7	&70.9	&-& 0.0&	12.2&	\textbf{18.2}&	0.0&	\textbf{17.6}&	\textbf{62.9}\\
OLN-SSOS (Ours) &3.6	&15.5	&17.8	&15.7	&70.9	&-& 0.0&	12.2&	\textbf{18.2}&	0.0&	\textbf{17.6}&	\textbf{62.9}\\
% OLN-VOS Box $k=20$(Ours) &3.8	&15.7	&18.0	&15.9	&70.2	&-& 3.2&	5.2&	6.6&	0.2&	11.4&	2.2\\
% OLN-FFS Box $k=5$ (Ours) &3.9	&16.8	&19.4	&17.3	&70.5	&-& 4.2&	\textbf{12.3}&	12.8&	2.6&	9.2&	50.2 \\
OLN-FFS (Ours) &3.9	&16.8	&19.4	&17.3	&70.5	&-& 4.2&	\textbf{12.3}&	12.8&	2.6&	9.2&	50.2 \\ \hline
% OLN-FFS Box $k=10$ (Ours) &4.0	&16.3	&18.8	&16.7	&69.8	&-& 2.7&	5.2&	8.1&	3.4&	10.1&	10.7\\
% OLN-FFS Box $k=20$ (Ours) &3.8	&15.8	&17.9	&15.9	&65.8	&-& 2.0&	4.1&	10.4&	\textbf{4.5}&	6.4&	39.5\\ \hline
\end{tabular}%
}
\renewcommand{\arraystretch}{1}
\end{table}

==> tables/results_sixray10.tex <==
\begin{table}[t]
\centering
\caption{Anomaly detection metrics for the SIXRay10 dataset.}
\label{tab:sixray10_results}
\resizebox{\linewidth}{!}{%
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{|l|cccccc|cccccc|}
\hline
 & \multicolumn{6}{|c|}{In-distribution Test Set} & \multicolumn{6}{|c|}{OoD Test Set} \\ \hline
\textbf{Method} & \textbf{AR@1} & \textbf{AR@10} & \textbf{AR@100} & \textbf{AR@S} & \textbf{AR@M} & \textbf{AR@L} & \textbf{AR@1} & \textbf{AR@10} & \textbf{AR@100} & \textbf{AR@S} & \textbf{AR@M} & \textbf{AR@L} \\ \hline
SIREN \cite{du2022siren}  & 47.8&	63.3&	63.7&	10.0	&62.8&	64.7 & 0.8&	0.8&	0.8&	0.0	&0.0&	0.9\\
VOS \cite{du2022vos}   &48.2	&63.6&	63.6&	0.0&	62.2&	65.0 & 0.0	&0.1&	0.1&	0.0&	0.0&	0.2\\
FFS  \cite{kumar2023normalizing}  &\textbf{49.2}&	\textbf{65.4}&	\textbf{65.4}&	60.0&	\textbf{65.1}&	\textbf{65.8} & 0.8&	0.8&	0.8&	0.0&	0.0&	1.0\\
% OLN-VOS Box $k=5$ (Ours) &29.9	&52.2&	57.4&	50.0&	58.1&	57.0& 8.0&	20.9&	30.5&	47.5&	27.8&	30.6\\
% OLN-VOS Box $k=10$(Ours) &31.3&	51.7&	56.6&	30.0&	56.9&	56.6& 5.2&	12.6&	18.4&	32.5&	27.5&	17.3\\
% OLN-VOS Box $k=20$(Ours) &28.0&	49.2&	55.2&	\textbf{70.0}&	56.4&	54.4& 10.7&	25.8&	35.3&	55.0&	34.2&	35.3\\
OLN-SSOS (Ours) &28.0&	49.2&	55.2&	\textbf{70.0}&	56.4&	54.4& 10.7&	25.8&	35.3&	55.0&	34.2&	35.3\\
% OLN-FFS Box $k=5$ (Ours) &30.9&	52.9&	57.2&	60.0&	57.8&	56.8& 4.6&	13.5&	18.5&	15.0&	16.4&	18.8\\
% OLN-FFS Box $k=10$ (Ours) &31.0&	51.5&	56.5&	50.0&	57.6&	55.9& 9.8&	23.5&	33.0&	\textbf{57.5}&	\textbf{35.1}&	32.6\\
% OLN-FFS Box $k=20$ (Ours) &29.8&	50.4&	55.1&	30.0&	55.3&	55.1& \textbf{12.1}&	\textbf{27.3}&	\textbf{35.6}&	40.0&	32.0&	\textbf{36.0}\\ \hline
OLN-FFS (Ours) &29.8&	50.4&	55.1&	30.0&	55.3&	55.1& \textbf{12.1}&	\textbf{27.3}&	\textbf{35.6}&	40.0&	32.0&	\textbf{36.0}\\ \hline
\end{tabular}%
}
\renewcommand{\arraystretch}{1}
\end{table}

==> tables/roadanomaly21.tex <==

\FloatBarrier
\begin{table*}[!htb]
    \centering
    \begin{tabular}{|l||c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline  
          &&  &  \multicolumn{3}{|c|}{Pixel-level}&    &&\multicolumn{12}{|c|}{Component-level}\\ \hline  
          &&  &  \multicolumn{3}{|c|}{Anomaly scores}&    &&&  &  \multicolumn{3}{|c|}{$\tau$ = 0.25}&  \multicolumn{3}{|c|}{$\tau$ = 0.50}&  \multicolumn{3}{|c|}{$\tau$ = 0.75}& \\ \hline  
          &k& ep&AuPRC  &  FPR$_{95}$&$F_{1}$  &  k&ep&sIoU   &PPV   &FN   &FP   &$F_{1}$ &  FN   &  FP   &  $F_{1}$ &  FN   &  FP   &  $F_{1}$ & $\overline{F_{1}}$ \\ \hline  
          vos&5&12   &  57.2&  22.5&  61.2&    5&18&58.8&  13.2& \textbf{1} &  66& 30.9&  5&  69&  22.9&  12&  74&  8.5& 21.5\\ \hline  
          vos-ffs&40&  58&  53.7&  \textbf{17.2}&  65.1&    40&59&60.1&  18.8&  \textbf{1}&  56& 34.5&  6&  60&  23.3& \textbf{11}&  61&  12.3& 24.9\\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline 
    \end{tabular}
    \caption{SMIYC-Anomaly Track-val}
    \label{tab:my_label}
\end{table*}

\begin{figure}[p]
\centering
\includegraphics[width=\linewidth]{figures/roadanomaly_val.png}
\end{figure}

\FloatBarrier

\FloatBarrier
text
\begin{table*}[h!]
    \centering
    \begin{tabular}{|l||c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline  
          &&  &  \multicolumn{3}{|c|}{Pixel-level}&    &&\multicolumn{12}{|c|}{Component-level}\\ \hline  
          &&  &  \multicolumn{3}{|c|}{Anomaly scores}&    &&&  &  \multicolumn{3}{|c|}{$\tau$ = 0.25}&  \multicolumn{3}{|c|}{$\tau$ = 0.50}&  \multicolumn{3}{|c|}{$\tau$ = 0.75}& \\ \hline  
          &k& ep&AuPRC  &  FPR$_{95}$&$F_{1}$  &  k&ep&sIoU   &PPV   &FN   &FP   &$F_{1}$ &  FN   &  FP   &  $F_{1}$ &  FN   &  FP   &  $F_{1}$ & $\overline{F_{1}}$ \\ \hline  
          vos&5&9&  86.1&  21.1& \textbf{90.8}  &    5&6& \textbf{57.6}&  19.9&  14&  106& 34.1&  14&  106&  34.1&  20&  110&  27.8& 32.7\\ \hline  
          vos-ffs&5&  4&  77.1&  29.8&  85.4&    k&4&67.1&  47.5& \textbf{7}  &  32& 66.1& \textbf{8} &  33&  64.3& \textbf{18} &  38&  49.1& 60.4\\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline 
    \end{tabular}
    \caption{SMIYC-Obstacle Track-val}
    \label{tab:my_label}
\end{table*}

\FloatBarrier
\FloatBarrier
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figures/roadobstacle_val.png}
\end{figure}
\FloatBarrier

==> tables/smiyc_test.tex <==


\FloatBarrier
\begin{table*}[!htb]
    \centering
    \begin{tabular}{|l||c|c|c|c|c|l|l|c|c|c|c|} \hline  
          &&\multicolumn{5}{|c|}{Anomaly Track}&\multicolumn{5}{|c|}{Obstacle Track}\\ \hline  
          &&  AP&  FPR&  sIoU gt&  PPV&    mean F1&AP&FPR&  sIoU gt&  PPV&  mean F1\\ \hline  
          &&  59.1&  20.4&  47.9&  19.8&    23.3&42.7&39.0&  9.1&  87.7&  57.2\\ \hline 
    \end{tabular}
    \caption{SMIYC-Anomaly Track-test}
    \label{tab:my_label}
\end{table*}



\begin{figure}[p]
\centering
\includegraphics[width=\linewidth]{figures/smiyc_test.png}
\end{figure}

\FloatBarrier



==> tables/smiyc_testdetails.tex <==
\FloatBarrier
test
\begin{table*}[h!]
    \centering
    \begin{tabular}{|l|c|c|c|c|c|l|l|c|c|c|c|c|c|c|c|c|c|c|c|} \hline  
          &&  &  \multicolumn{3}{|c|}{Pixel-level}&    &&\multicolumn{12}{|c|}{Component-level}\\ \hline  
          &&  &  \multicolumn{3}{|c|}{Anomaly scores}&    &&&  &  \multicolumn{3}{|c|}{$\tau$ = 0.25}&  \multicolumn{3}{|c|}{$\tau$ = 0.50}&  \multicolumn{3}{|c|}{$\tau$ = 0.75}& \\ \hline  
          &k& ep&AuPRC  &  FPR$_{95}$&$F_{1}$  &  k&ep&sIoU   &PPV   &FN   &FP   &$F_{1}$ &  FN   &  FP   &  $F_{1}$ &  FN   &  FP   &  $F_{1}$ & $\overline{F_{1}}$ \\ \hline 
 & \multicolumn{18}{|c|}{RoadAnomaly21 }&\\\hline \hline  
          &&&  59.1&  20.4&  67.4&    &&47.9&  19.8&  78&  748& 30.8&  119&  774&  24.3&  192&  820&  12.2& 23.3\\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline  
          &\multicolumn{18}{|c|}{RoadObstacle21}& \\ \hline  
          &&  &  42.7&  39.0&  57.2&    &&9.1&  87.7&  346&  1& 19.5&  350&  4&  17.7&  354&  6&  15.9& 17.6\\ \hline  
          &&  &  &  &  &    &&&  &  &  & &  &  &  &  &  &  & \\ \hline 
    \end{tabular}
    \caption{SMIYC-Anomaly Track-testdetails}
    \label{tab:my_label}
\end{table*}




\FloatBarrier
\begin{figure}[p]
\centering
\includegraphics[width=\linewidth]{figures/smiyc_testdetails.png}
\end{figure}

\FloatBarrier
